Age-Optimal Information Updates in Multihop Networks

The problem of reducing the age-of-information has been extensively studied in the single-hop networks. In this paper, we minimize the age-of-information in general multihop networks. If the packet transmission times over the network links are exponentially distributed, we prove that a preemptive Last Generated First Served (LGFS) policy results in smaller age processes at all nodes of the network (in a stochastic ordering sense) than any other causal policy. In addition, for arbitrary general distributions of packet transmission times, the non-preemptive LGFS policy is shown to minimize the age processes at all nodes of the network among all non-preemptive work-conserving policies (again in a stochastic ordering sense). It is surprising that such simple policies can achieve optimality of the joint distribution of the age processes at all nodes even under arbitrary network topologies, as well as arbitrary packet generation and arrival times. These optimality results not only hold for the age processes, but also for any non-decreasing functional of the age processes.

==> sections/NWU.tex <==
\section{NWU Service Time Distribution}
In this section, we consider a more general service time distribution, which is New-Worse than Used (NWU) service time distribution. We also consider  in order arrival packets. In this case, the optimal policy is preemptive LGFS (policy $P$) (since the arrivals are in order, LCFS policy and LGFS policy have the same age performance), which is depicted in Algorithm \ref{alg1}. We next show that the preemptive LGFS policy is age-optimal in case of NWU service time distribution. 
\begin{theorem}\label{thmNWU}
If the packet service times are NWU and \emph{i.i.d.} across time and servers, then for all packet generation and arrival time sequence $a_1, a_2, \ldots$, where $a_1\leq a_2\leq \ldots$,  and all queue sizes $B$, the preemptive LGFS policy is age-optimal.
\end{theorem}

To prove Theorem \ref{thmNWU}, we need to define the completion time of a packet as following:
Define $c_{i,\pi}$ as the completion time of the packet with time stamp $s_i$ under policy $\pi$. Without loss of generality, let $y_l$ and $y_k$ denote the packets with time stamps $s_l$ and $s_k$, respectively, where $s_k\geq s_l$. If the packet $y_l$ is preempted by the packet $y_k$ or the packet $y_k$ is delivered while the packet $y_l$ is being processed, then we have 
\begin{equation*}
c_{l,\pi}=c_{k,\pi}.
\end{equation*}  

The key step in the proof of Theorem \ref{thmNWU} is the following lemma, where we compare policy $P$ with any work-conserving policy $\pi \in \Pi_{wc}$.

\begin{lemma}\label{lemNWU1}
suppose that, for a given time instant $t \in [0, \infty)$, there exist $n$ packets arrived to the system. Then, for any given sequence of time stamps $(s_1, \ldots, s_n)$ of the arrived packets, where $s_1\leq \ldots\leq s_n$, we have
\begin{equation}\label{lawNWU_1}
c_{i,P}\leq_{\text{st}} c_{i,\pi},  \quad \forall i=1,\ldots,n,
\end{equation}
for all $\pi\in\Pi_{wc}$.
\end{lemma}

\begin{proof}
See Appendix~\ref{Appendix_F}.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thmNWU}]
Since the age is an increasing function of the packets completion time. As a result, Lemma \ref{lemNWU1} implies
\begin{equation}
\begin{split}
\{\Delta_{P}(t), t\in[0,\infty)\}\!\!\leq_{\text{st}} \!\!\{\Delta_{\pi}(t), t\in[0,\infty)\},~ \forall \pi\in\Pi_{wc}.\nonumber
 \end{split}
\end{equation}
Finally, since the service times are \emph{i.i.d.} across time and servers, service idling only increases the waiting time of the packet in the system. Therefore, the age under non-work-conserving policies will be greater. As a result, we have 
\begin{equation}
\begin{split}
 \!\!\!\!\!\!\!\{\Delta_{P}(t),  t\in[0,\infty)\}\leq_{\text{st}} \{\Delta_{\pi}(t), t\in[0,\infty)\}, \forall \pi\in\Pi.\nonumber
 \end{split}
\end{equation}
This completes the proof.
\end{proof}






%The proof of this Theorem is similar to the proof of Theorem \ref{thm1}. The proof idea is that, the preemptive LGFS policy starts serving the freshest packet before any other policy. The proof details are provided in Appendix~\ref{Appendix_F}.


==> sections/Near_age_optimality.tex <==
\section{Near Age-optimality Results}\label{nao}
\begin{figure}
\includegraphics[scale=0.5]{figure/sys_model2.eps}
\centering
\caption{ Information updates over a multihop network, where each node in the network (except the gateway) is restricted to receive data from only one node.}\label{Fig:sysMod2}
\vspace{-0.3cm}
\end{figure}

While the policy space being considered in Theorem \ref{thm1} (for exponential transmission distributions) is very general, the policy space considered in Theorem \ref{thm2} (for general transmission distributions) is restricted to only work-conserving policies. The next question we answer is whether for an important class of distributions that are more general than exponential, optimality or near-optimality can be achieved without the work-conserving policy space restriction. We consider the set of all non-preemptive policies, denoted by $\Pi_{np}\subset\Pi$. We propose non-preemptive LGFS policy and show that it is within three times of the optimum for minimizing the average age of all nodes in the network. However, we are able to prove this result for a somewhat more restrictive network than the general topology  $\mathcal{G(V, L)}$. The network here is represented by a directed graph $\mathcal{G'}(\mathcal{V},\mathcal{L})$, in which each node $i\in \{1,2, \ldots,N-1\}$ is allowed to receive data from only one node, as shown in Fig. \ref{Fig:sysMod2}. Each link in the network maintains a queue with infinite buffer size, i.e., $B_{ij}=\infty$ for all $(i,j)\in \mathcal{L}$. The packet transmission times are assumed to be \emph{i.i.d.} across time and links. We consider the classes of New-Better-than-Used (NBU) packet transmission time distributions, which are defined as follows.\\

 \noindent \textbf{Definition 4.} \textbf{New-Better-than-Used distributions:} Consider a non-negative random variable $X$ with complementary cumulative distribution function (CDF) $\bar{F}(x)=\mathbb{P}[X>x]$. Then, $X$ is \textbf{New-Better-than-Used (NBU)} if for all $t,\tau\geq0$
\begin{equation}\label{NBU_Inequality}
\bar{F}(\tau +t)\leq \bar{F}(\tau)\bar{F}(t).
\end{equation} 
In practice, NBU distributions include constant transmission time, (shifted) exponential distribution, geometrical distribution, Erlang distribution, etc. 

Define a set of parameters $\mathcal{I}'=\{n,(s_i, a_{i0})_{i=1}^{n}, \mathcal{G'(V, L)}\}$. Then, the age performance of non-preemptive LGFS policy among the policies in $\Pi_{np}$ is characterized in the following theorem.
\begin{theorem}\label{thm3}
Suppose that the packet transmission times are NBU and \emph{i.i.d.} across time and links, and $B_{ij}=\infty$ for all $(i,j)\in\mathcal{L}$, then for all $\mathcal{I}'$ such that the packet generation process $(s_1, s_2, \ldots)$ is a regenerative process
\begin{align*}
\min_{\pi\in\Pi_{np}} \mathbf{\bar{\Delta}}_{\pi}\leq \mathbf{\bar{\Delta}}_{\text{non-prmp-LGFS}}\leq 3\min_{\pi\in\Pi_{np}} \mathbf{\bar{\Delta}}_{\pi}, 
\end{align*}
where $\mathbf{\bar{\Delta}}_\pi=\left(\bar{\Delta}_{0,\pi}, \bar{\Delta}_{1,\pi}, \ldots, \bar{\Delta}_{N-1,\pi}\right)$, and $\bar{\Delta}_{j,\pi}=\lim_{T\rightarrow\infty}\frac{\int_0^{T} \Delta_{j,\pi}(t)dt}{T}$ is the average age at node $j$ under policy $\pi$.
\end{theorem}

\begin{proof}
We provide a proof sketch of Theorem \ref{thm3}. We will prove this theorem in three steps: in \emph{Step 1}, we will construct a virtual policy which provides an age lower bound of $\{\Delta_j(t), t\in [0,\infty)\}$ at each node $j\in\mathcal{V}$; in \emph{Step 2}, we prove that the constructed virtual policy is age optimal at each node of the network among the policies in $\Pi_{np}$; in \emph{Step 3}, we will evaluate the age gap between the age lower bound and the average age of non-preemptive LGFS policy. 
\ifreport
See Appendix~\ref{Appendix_C} for the details.
\else
See our technical report for the details.\fi
\end{proof}

%
%\begin{align*}
%\min_{\pi\in\Pi_{np}} \bar{\Delta}_{j,\pi}\leq \bar{\Delta}_{j, \text{non-prmp-LGFS}}\leq\min_{\pi\in\Pi_{np}} \bar{\Delta}_{j,\pi} + (2k-1)\mathbb{E}(X), 
%\end{align*}
%or equivalently, ,

%In this section, we focus on the network consisting of $N$ nodes, where  We represent this network by a directed graph $\mathcal{G'}(\mathcal{V},\mathcal{L})$, where $\mathcal{V}$ is the set of nodes and $\mathcal{L}$ is the set of links. Let $H_k$ denote the set of nodes in the $k$-th hop (that are separated by $k$ links from node $0$), where node $0$ is always considered to be in $H_0$.

%We define the competitive ratio of a policy $\beta$ as the maximum ratio of the achieved average age of all nodes in the network for policy $\beta$ to the achieved average age of all nodes in the network for an optimal virtual policy.
